LongRoPE2: Near-Lossless LLM Context Window Scaling

LongRoPE2 is a novel approach that extends the effective context window of pre-trained large language models (LLMs) to the target length, while preserving the performance on the original shorter context window. This is achieved by three contributions: (1) a hypothesis that insufficient training in higher RoPE dimensions contributes to the persistent out-of-distribution (OOD) issues observed in existing methods; (2) an effective RoPE rescaling algorithm that adopts evolutionary search guided by "needle-driven" perplexity to address the insufficient training problem; (3) a mixed context window training approach that fine-tunes model weights to adopt rescaled RoPE for long-context sequences while preserving the short-context performance with the original RoPE. Extensive experiments on LLaMA3-8B and Phi3-mini-3.8B across various benchmarks validate the hypothesis and demonstrate the effectiveness of LongRoPE2. Remarkably, LongRoPE2 extends LLaMA3-8B to achieve a 128K effective context length while retaining over 98.5% of short-context performance, using only 10B tokens -- 80x fewer than Meta's approach, which fails to reach the target effective context length. Code will be available at https://github.com/microsoft/LongRoPE.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method1.tex <==


\section{{\sysname} Methodology}

\subsection{Theoretical Analysis}
\noindent\textbf{RoPE in attention long-term decay theory}. To address these challenges, we revisit the role of RoPE in transformer architecture and identify a key property that should be factored into RoPE rescaling for long context extension.  While RoPE is well-known for its simple and effective encoding of position information, it also introduces a crucial long-term decay property. Specifically, the upper bound of  attention inner production will decay when the relative position increase as shown in Fig.~\ref{fig:ropedecay1}. This property of RoPE makes the model attend more to closer tokens, serving as valuable prior knowledge for the attention mechanism. 
Let $h_l=\mathbf{q}_{[2l:2l+1]}\mathbf{k}^*_{[2l:2l+1]}$, $S_l=\sum_{j=0}^{l-1}e^{i(m-n)\theta_j}$, the upper bound of the attention inner product in Eq.~\ref{eq:attention-1} can be written as follows: 
\begin{gather}
	\label{eq: attentiondecay1}
	\mathbf{q}^T_m\mathbf{k}_n \le \left(\max_{l}|h_{l+1}-h_l|\right)\sum_{l=0}^{d/2-1}|S_{l+1}|, \text{where}\quad  S_l=\sum_{j=0}^{l-1}e^{i(m-n)\theta_j}
\end{gather}
Then, as introduced in the original RoPE~\citep{rope}, the value of $\frac{1}{d/2}\sum_{l=1}^{d/2}|S_l|$ can be used as a measure of attention inner product decay with the relative distance $m-n$. Fig.~\ref{fig:ropedecay1} shows the long-term decay curve of this upper bound across different scales of relative position distances. 

Surprisingly, we find that this theory helps explain RoPE rescaling for context window extension. 
 \textbf{(1)} In the example of Phi3-mini, within the pretrained 2k context length, there is a clear decay property as shown in Fig.~\ref{fig:ropedecay1}(b). However, when directly extrapolating to 128k, the attention inner product beyond 2k no longer exhibits this decay, making it difficult for attention to distinguish tokens at long distances. 
Fortunately, applying RoPE rescaling methods like NTK and LongRoPE restores the long-term decay trend, allowing self-attention to effectively distinguish tokens within the 128k context window.  \textbf{(2)} Fig.~\ref{fig:ropedecay1}(a) zooms in the decay of different approaches at short relative distance, where the current token pays more attention to the tokens at these distances. NTK and LongRoPE match the pretained model's short-term decay trend. However, YaRN exhibits an anomaly between relative distances of 20-40, where attention scores increase rather than decay, leading  self-attention assigning more weight to mid-range distances than to very close ones (e.g., 0-20). 

The above analysis highlights the need to preserve the attention decay property in RoPE rescaling  for long context extension. However, current approaches like YaRN can disrupt this critical property. This raises the question: how can we preserve this property during RoPE rescaling? While this property is difficult to solve analytically, we draw inspiration from NTK's theta scaling: using a larger theta base value naturally preserves the property within long context window. This translates to applying monotonically increasing scaling factors from lower to higher RoPE dimensions (the proof is provided in appendix). We thus derive the following theorem: 

\noindent\textbf{Theorem 1}. \textit{After extending a pre-trained LLM to a long context window,  the upper bound of attention inner product must maintain its long-term decay property. This is can be ensured by applying the following constraint to RoPE rescaling factors:}
\begin{gather}
	\label{eq:theory}
	\lambda_0<\lambda_1<...<\lambda_i < \lambda_{i+1}<...<\lambda_{d/2-1}  
\end{gather}
This theorem can be viewed as a stricter version of NTK theory, which YaRN does not satisfy.
 Specifically, it addresses Question \textit{1} in Section~\ref{sec:challenegs}. \textit{Although lower RoPE dimensions do not violate RoPE OOD theory or NTK theory, they still need to be rescaled to meet Theorem 1 and maintain the attention decay property.}
Our analysis reveals that YaRN's setting of scaling factors for high-frequency RoPE dimensions (i.e., $\lambda_i=1, i\le d_\text{high\_freq}$) to 1 causes the anomalous increase in attention upper bound at short-term distances.
NTK naturally adheres to this theorem, while LongRoPE, due to its monotonically non-decreasing scaling factors, does not strictly fulfill it.





\noindent\textbf{The actual RoPE  periods in higher dimensions are shorter than theoretical values}. Another fundamental question  is: why are scaling factors beyond the critical dimension required to be larger than the theoretical value $s$? Our hypothesis is that these higher dimensions do not receive sufficient training during pretraining, resulting in shorter rotation periods than the theoretical values as expected. 

Specifically, $\theta_i (m-n)$ represents the RoPE values at the $i^{th}$ dimension during pre-training. Higher rotation frequencies $\theta_i$ in lower dimensions enable them to complete their full rotation periods easily.  For instance,  the 8$^{th}$ dimension requires sufficient training with token relative distances of $m-n=24$ to complete one full period (see Fig.~\ref{fig:ropeperiod}). In contrast, the critical 31$^{st}$ $consine$ dimension requires relative distances of $m-n=2048$  to complete its period. While token pairs with relative distances of 24 are common in the  pretraining corpus, long token dependencies like 2048 are relatively rare in real-world data. Moreover, 2048 corresponds to Phi3's pretrained context window size. This explains why larger scaling factors than $s$ in higher RoPE dimensions usually achieve better performance. Then, we propose Hypothesis 1 as follows: 

\noindent\textbf{Hypothesis 1}. \textit{Insufficient training in higher RoPE dimensions results in actual RoPE periods being shorter than the theoretical values of $\frac{2\pi}{\theta_i}$. Consequently, this requires larger scaling factors in these dimensions, and the actual critical dimension index is smaller than the theoretical value in Eq.~\ref{eq:cd}.}





\subsection{Search}

\noindent\textbf{Synthetic long data to guide the search}. 

\noindent\textbf{Search for practical critical dimension}.

\noindent\textbf{}




\subsection{Mixed Context Window Training for Short Performance Recovery}

\noindent\textbf{Mixed Context Windows Training}

1. per batch data must be same length 


efficiency 

loss: 

2. 

shuffle: 


==> rw.tex <==
\section{Background}

\noindent\textbf{Rotary Position Embedding (RoPE)}. Transformer models require explicit positional information, often in the form of position embedding, to represent the order of input tokens.  Our work builds on the Rotary  Position Embedding (RoPE)~\citep{rope}, a position encoding technique widely used in modern LLMs.  Formally, for a token at position indices $n$, the positional information is encoded using a trigonometric rotation matrix, which can be simplified as follows:
%\vspace{-1ex}
\begin{equation}
%	\fontsize{7.8}{7.8} \selectfont
	\label{eq:rope}
	\left[ cos(n\theta_0), sin(n\theta_0), cos(n\theta_1), \cdot\cdot\cdot, cos(n\theta_{d/2-1}), sin(n\theta_{d/2-1}) \right]   
\end{equation}
Here, $d$ is the embedding dimension size, 
 and $\theta_i=\theta^{-2i/d}$ is the rotation frequencies in the $i^{th}$ dimension, where the default base value of $\theta$ is 10000. 
 
In Equation~\ref{eq:rope}, RoPE for a token at position $n$ is encoded by applying a rotary angle $n\theta_i$ to each dimension using trigonometric function.  This positional information is then added to the query and key vectors before attention, which results in  the attention being a function of the relative distance between tokens. Specifically, for two positions, $m$ and $n$, its self-attentions score computes $cos((m-n)\theta_i)$ and $sin((m-n)\theta_i)$, where $m-n$ is their relative positional distance. 


% this results in  the attention being a function of the relative distance between tokens. Specifically, for two position indices $m$ and $n$,  its self-attention score computes $cos((m-n)\theta_i)$ and $sin((m-n)\theta_i)$, which means that the attention score is only dependent on relative position $m-n$ rather than their absolute position values. 


Despite its effectiveness, RoPE, like other position encodings, faces challenges in context length extrapolation.  In particular, when the input sequence length exceeds the predefined context window, the perplexity can shoot up to very high numbers (i.e., $>10^3$), comparable to untrained models. This happens because longer sequences introduce out-of-distribution relative rotation angle $(m-n)\theta_i$, which causes catastrophic values in attention computation~\citep{pi,han2023lminfinite}. 




%where $d$ is the RoPE embedding dimension, ($n\theta_i$) is the rotary angle in the $i^{th}$ dimension for the token at position $n$, and $\theta_i=\theta^{-2i/d}$ represents the rotation frequencies. In RoPE, the default base value of $\theta$ is 10000. 



\noindent\textbf{RoPE Rescaling for Context Window Extension}.  To address this OOD issue, recent works~\citep{pi,ntk,yarn,longrope} show that the context window of a pre-trained LLM can be extended by rescaling RoPE rotation angles. The insight is to downscale new position indices to fit within the pre-trained range. 
Representative methods include PI~\citep{pi}, NTK~\citep{ntk}, YaRN~\citep{yarn} and LongRoPE~\citep{longrope}.  Each offers a different way to calculate the rescaling factors. Formally, let  $\beta=\theta^{2/d}$ and $\lambda_i$ be the rescaling factor for the $i^{th}$ RoPE dimension, we unify these rescaled RoPE methods as follows:
\begin{equation}	
	\fontsize{8}{8} \selectfont
	\label{eq:rescale_rope}
	\begin{aligned}
		\left[cos\left(\frac{n}{\lambda_0(\beta^0)}\right), sin \left(\frac{n}{\lambda_0(\beta^0)}\right), cos\left(\frac{n}{\lambda_1(\beta^1)}\right), \cdot\cdot\cdot,  cos\left(\frac{n}{\lambda_i(\beta^i)}\right),  \cdot\cdot\cdot,  sin \left(\frac{n}{\lambda_{d/2-1}(\beta^{d/2-1})}\right) \right]   
	\end{aligned}
\end{equation}





\noindent\textit{Linear PI}. The value of $\lambda_i$ is typically dependent on the  target context window extension ratio $s$. For instance, PI proposes linear positional interpolation, where the rotation angles  are linearly reduced by $\lambda_i=s$ across all RoPE dimensions. However, this approach "crowds" the positional information,  making it difficult for the model to distinguish closely positioned tokens. 




\noindent\textit{NTK and YaRN}. To mitigate this issue, NTK and YaRN propose uniformly rescaling the RoPE dimensions based on  Neural Tangent Kernel theory~\citep{jacot2018neural,tancik2020fourier}. 
 The idea is that neural networks are difficult to learn high-frequency features, and direct interpolation can affect the high-frequency positional information. As a result, these approaches apply less interpolation to lower (high-frequency) RoPE dimensions and larger rescaling factors to higher (lower-frequency) dimensions to achieve more interpolation. Specifically, NTK proposes to increase the original RoPE base value $\theta$ using a formula $\lambda_i=s^{2i/(d-2)}$~\citep{ntk}.  YaRN suggests dividing RoPE dimensions into three groups: higher-frequency dimensions use direct extrapolation ($\lambda_i=1$),  lower-frequency dimensions use PI ($\lambda_i=s$), and dimensions that fall in-between employs the NTK. 
 
 %ntk:  $\theta_i=(k\theta)^{-2i/d}$, $k=(s)^{2/(d-2)}$

 \noindent\textit{Non-uniformities and LongRoPE}. 
 Despite their simplicity, NTK and YaRN require expert  tuning to configure the optimal rescaling factors, making them challenging to apply in practical LLM context window extensions. Recent study~\citep{men2024base} suggest that the current rescaled $\theta$ base in NTK is insufficient to achieved the claimed context window and needs to be larger.  However, setting the optimal value is difficult, and using a significantly larger NTK rescaled $\theta$ can negatively impact performance.
For YaRN, success heavily depends on how RoPE dimensions are grouped. However, the grouping tuned for an LLM can become ineffective for new LLMs with a different number of RoPE dimensions. 
  Later, LongRoPE~\citep{longrope} revisited these approaches and  identified subtle non-uniformities in RoPE dimensions that current methods fail to address effectively. Based on this, LongRoPE propose an efficient evolution search algorithm to automatically achieve better RoPE rescaling solutions. 
 


\begin{table}[ht]
	\centering
	\small
	\caption{Summary of RoPE rescaling methods.}
	\label{tbl:roperescaling}
	\resizebox{0.7\textwidth}{!}{	\begin{tabular}
			{ccc}
			\toprule
		&	Method &   Rescaling factors\\
		\hline
			PI &Linear Rescaling& \\
			NTK &Base value rescaling& \\
			YaRN &Group-wise Rescaling& \\
			LongRoPE &Per-dimension non-uniform Rescaling& \\
			{\sysname} & Per-dimension non-uniform Rescaling&\\
			\hline
			\end{tabular}}
	\end{table}
	
\lz{plot a figure to show the per-dimension scaling factors} 


\noindent\textbf{Long Context Fine-tuning}.  To achieve reliable performance in practical long context applications, a continuous pre-training stage is typically used to adapt model weights to the rescaled RoPE in state-of-the-art long context LLMs~\citep{llama3.1,qwen2,chatglm,deepseekcoder}.  Specifically, a target context window size is predefined, and data is chunked to match this size. During fine-tuning, all data lengths conform to this predefined context window size. 

\noindent\textbf{Short Performance Recovery}. A well-known issue is that an extended long context LLM loses  performance at the original context window, which poses a significant challenge during practical LLM training. To address this issue, LLaMA3.1~\citep{llama3.1} applies a gradual context window extension over six stages (from 8k to 128k). However, this significantly increases training complexity and costs. LongRoPE proposes using a dedicated short scaling factor specially for handling inference within the original context window size. 



==> rw1.tex <==
\section{Related Works}
